Measuring the robustness of Gaussian processes to kernel choice

Gaussian processes (GPs) are used to make medical and scientific decisions, including in cardiac care and monitoring of atmospheric carbon dioxide levels. Notably, the choice of GP kernel is often somewhat arbitrary. In particular, uncountably many kernels typically align with qualitative prior knowledge (e.g.\ function smoothness or stationarity). But in practice, data analysts choose among a handful of convenient standard kernels (e.g.\ squared exponential). In the present work, we ask: Would decisions made with a GP differ under other, qualitatively interchangeable kernels? We show how to answer this question by solving a constrained optimization problem over a finite-dimensional space. We can then use standard optimizers to identify substantive changes in relevant decisions made with a GP. We demonstrate in both synthetic and real-world examples that decisions made with a GP can exhibit non-robustness to kernel choice, even when prior draws are qualitatively interchangeable to a user.

==> experiments.tex <==
\section{Experiments}
\subsection{Toy experiments?}
\begin{enumerate}
	\item Objective: Establish that our test doesn't always say things are not robust.
\end{enumerate}

\subsection{Stationary neighborhoods through spectral construction}
\begin{enumerate}
	\item MaunaLoa --- 1D example of predictive robustness (toy?)
	\item Heartrate --- 1D example of predictive robustness (real world)
	\item Light curves --- 1D example of inferential robustness (real world)
\end{enumerate}

\subsection{Non stationary neighborhoods through input warping}
\begin{enumerate}
	\item MaunaLoa --- 1D example of predictive robustness but the neighborhood now includes non-stationary kernels.
	\item Neural Kernels on MNIST --- High dimensional example.  	
\end{enumerate}


Figure~\ref{fig:mauna_loa_example} is a placeholder


\begin{figure}[H]
\centering
\includegraphics[width = 0.95\linewidth]{figures/mauna_loa_example.png}
\caption{Placeholder image of Mauna Loa fit}
\label{fig:mauna_loa_example}
\end{figure}

==> input_warping.tex <==
%!TEX root = neurips_2021.tex
\label{sec:non-stationary}
%
\begin{algorithm}
    \caption{Objective for non-stationary kernels \wts{Ideally: FIX NUMBERING and naming... should be ``Constraint Set 2'' not ``Algorithm 4''}}
    \begin{algorithmic}[1]
    \label{constraintSet:nonStationary}
    \State \textbf{Input:} Regularizer grid points $x_1, \dots, x_M$, regularizer strength $\eps > 0$, neural network weights $w \in \R^D$.
    \State Define neural network $h(x; w)$ parameterized by weights $w$.
    \State Define $k_1(x_1, x_2) := k_0(x_1 + h(x_1; w), x_2 + h(x_2; w))$.
    \State \Return{$\lvert F^{\star}(k_1) - \Delta \rvert^{2} + \frac{1}{\eps} \frac{1}{M}\sum_{m=1}^M ||h(x_m, w)||_2^2$ }
    \end{algorithmic}
   \label{alg:non-stationary}
\end{algorithm} 
%
Up to this point, we have only considered stationary neighborhoods $K$ containing $k_0$. 
However, in many modeling problems, stationarity may only be a choice of convenience rather than a strong prior belief or there may be a strong prior belief of non-stationarity. In both cases it is natural to search for non-stationary perturbed kernels $\kperturb$. 
We extend our framework to this case by defining a non-stationary neighborhood $\Kns$ around $k_0$. While there are several methods for constructing non-stationary kernels, a particularly convenient technique for our purposes relies on input warping~\cite[Sec 4.2.3]{RasmussenWilliams2006}. Given a kernel $k_0$, a non-linear mapping $g$, we define a perturbed kernel $k(x_1, x_2) = k_0(g(x_1), g(x_2))$. 
This construction guarantees that the perturbed kernel $k$ is a kernel function as long as $k_0$ is a valid kernel. We set
$
g(x; w) := x + h(x; w), 
$
where $h: \R^D \rightarrow \R^D$ is a small neural network parameterized by a set of weights $w$. 
By controlling the magnitude of $h$, we can control the deviations from $k_0$.

We could optimize over the set of non-stationary kernels with respect to the weights $w$, under the constraint $\|h(x;w)\|_2^2 \leq \eps$. 
However, it is unclear how to enforce this constraint.
Instead, we select a grid of points $x_1, \dots, x_m \in \R^D$ and add a regularizer to our objective,
$
\frac{1}{\eps} \frac{1}{m}\sum_i ||h(x_i, w)||_2^2,
$
%
%\begin{equation}
%\hat{w} = \argmin_{w} \; \lvert F^{\star}(k(w)) - \Delta \rvert^{2} + \frac{1}{\eps} \frac{1}{m}\sum_i ||h(x_i, w)||_2 ,  
%\label{nonStationaryOpt}
%\end{equation}
%
where $\eps$ controls the regularization strength. 
While we would ideally regularize using the entire function $h$, we find using a grid of points to be computationally cheap, mathematically simple, and empirically effective.
We summarize our objective as a function of the network weights $w$  in \cref{constraintSet:nonStationary}.
Note also that we have also modified our objective to ensure it  is bounded.
Optimizing directly over $\Fstar(k(w))$ is not guaranteed to give a bounded objective; e.g.\ moving some direction in kernel space could give kernels infinitely far away from $k_0$ but also have an infinite value of $\Fstar(k(w))$.
Given the minimum $\hat w$ to the objective in \cref{constraintSet:nonStationary}, we set $\kperturb = k(\hat w)$.



==> math.tex <==
\newcommand{\nbor}{\mathcal{N}_\epsilon(k_0)}
\newcommand{\N}{\mathcal{N}} % caligraphic N for normal distribution
\newcommand{\GP}{\mathcal{GP}} % caligraphic GP for Gaussian process
\newcommand{\R}{\mathbb{R}} %blackboard R for reals
\newcommand{\Exp}{\mathbb{E}} % blackboard E for expectation
\newcommand{\Prob}{\mathbb{P}} % blackboard P for probability
\newcommand{\bx}{\bm{x}} % bold X for vector of inputs
\newcommand{\xtest}{\bx^{\star}} % star x for test input
\newcommand{\ftrain}{\bm{f}} % bold f for vector of training observations
\newcommand{\ftrainvec}{(f(\bx_{1}), \ldots, f(\bx_{N}))^{\top}} % vector of training observations
\newcommand{\ftest}{f^{\star}}
\newcommand{\Data}{\mathcal{D}}
\newcommand{\kperturb}{k_1}
\newcommand{\Fstar}{F^\star}
\newcommand{\bigChange}{\Delta}



% comment macros
\newcommand{\skd}[1]{\textcolor{blue}{\small [skd]: #1}}
\newcommand{\wts}[1]{\textcolor{red}{\small [wts]: #1}}
\newcommand{\tdn}[1]{\textcolor{purple}{\small [tdn]: #1}}

==> methods.tex <==
\section{Methods}
We begin with an overview of our approach,
\begin{enumerate}
\item Given a kernel $k_0$, define an $\epsilon$-set, $\nbor$, centered at $k_0$. The set $\nbor$ is restricted to valid kernel functions. 	
\item If there exists a $\tilde{k} \in \nbor$, such that a prediction or inference of interest under a GP model with $k_0$ and a GP model with $\tilde{k}$, differ by $\delta$ or more, then we deem $k_0$ not $(\epsilon, \delta)$ robust. 
\end{enumerate}

We now fill in details about how $\nbor$ is constructed and how we search for $\tilde{k} \in \nbor$. 



==> related-work.tex <==
\subsection{Related work}

%\paragraph{Robustness \& sensitivity}
%\skd{A small review of Bayesian robustness, local sensitivity. } 

Insofar as the covariance kernel is just a prior hyperparameter, our aims in this paper are similar in spirit to those pursued in a rich literature on Bayesian robustness and local sensitivity.
Specifically, \cite{Gustafson1996_local, Giordano2018_covariance, Liu2018_stickbreaking} carefully study how infinitesimal changes to finite-dimensional hyperparameters can affect posterior expectations.
The methods developed in those papers, however, are not as easy to apply to assess the sensitivity of more complex functions like quantiles to more general changes to the covariance kernel. 

Our goals are distinct from those pursued in the automated or flexible kernel discovery literature.
\cite{Duvenaud2013_compositional}, for instance, selects a kernel by iteratively searching over elementary combinations of simpler kernels.
\cite{Wilson2016_dkl}, on the other hand, increases the representational flexibility of elementary kernels by first transforming the inputs using a neural network.
\cite{WilsonAdams2013_sm} and \cite{Benton2019_function} instead model the spectral density of a $k$ with, respectively, a mixture of Gaussians and exponentiated GP. 
In all of these works, the goal was to adaptively identify a kernel from a flexible class that fits the data well.
Our focus, in contrast, is to construct a new kernel that (i) encodes similar prior beliefs to kernel --  elicited from real prior beliefs or adaptively identified -- while (ii) producing different posterior predictive inference. 

It is also important to note a distinction between our focus on prior perturbations and the existing literature on robust GPs, which is primarily concerned with assessing sensitivity to perturbations to the data.
\cite{Jylanki2011_student-t} and \cite{Ranjan2016_em}, for instance, reduce the influence of outlying observations in GP regression by replacing the conventional Gaussian noise model with heavier-tailed alternatives.
%Much of the work on robust GP regression, classification, and optimization concerns the behavior of a GP model under perturbations to the data. 
%First-order techniques like those in \cite{Giordano2018_covariance} can help diagnose the sensitivity of posterior expectations to infinitesimal perturbations of the learned kernel hyper-parameter.
%They cannot, however, be easily applied to assess the sensitivity of more complex functionals like quantiles to more general changes to the covariance kernel. 
%\paragraph{Robust GP modeling}
%Much of the work on robust GP regression, classification, and optimization concerns the behavior of a GP model under perturbations to the data. 
%For instance, to reduce the influence of outlying observations in GP regression, \cite{Jylanki2011_student-t} and \cite{Ranjan2016_em}, replace the conventional Gaussian noise model with heavier-tailed alternatives.
\cite{KimGhahramani2008_outlier} and \cite{Hernandez-Lobato2011_multiclass} similarly propose GP classifiers that respectively are robust to outliers and label noise.
A more recent line of work concerns potentially adversarial perturbations to a test point $\xtest.$
In the respective contexts of regression and optimization, \cite{Cardelli2019_aaai} and \cite{Bogunovic2018_optimization} carefully control the maximal change in the value of the latent function over a local neighborhood of $\xtest.$
For classification, \cite{Blaas2020_classification} similarly bounds the maximal and minimal values of the class probabilities in a neighborhood of $\xtest$ while \cite{Smith2019_vulnerability} instead bound the size of input perturbation required to change the label of a confidently classified test observation.

%\sg{I think it is probably useful to talk about related approaches for kernel learning and point out goals / methods are different, to ward off the lazy reviewer.}

%To the best of our knowledge, there has been comparatively less work seeking to assess sensitivity to perturbations of the assumed GP prior, which is our ultimate focus.
To the best of our knowledge, the only work that assesses sensitivity to kernel specification is \cite{WangJing2021_convergence}, which establishes optimal convergence rates for GP regression when the smoothness implied by the selected covariance kernel is misspecified. 
While interesting and important, their results do not provide insight into how kernel misspecification affects functionals like posterior predictive means or quantiles in finite samples, nor do they provide specific information about any given application.
